Deep Learning-Based Channel Extrapolation for Dual-Band Massive MIMO Systems

Future wireless communication systems will increasingly rely on the integration of millimeter wave (mmWave) and sub-6 GHz bands to meet heterogeneous demands on high-speed data transmission and extensive coverage. To fully exploit the benefits of mmWave bands in massive multiple-input multiple-output (MIMO) systems, highly accurate channel state information (CSI) is required. However, directly estimating the mmWave channel demands substantial pilot overhead due to the large CSI dimension and low signal-to-noise ratio (SNR) led by severe path loss and blockage attenuation. In this paper, we propose an efficient \textbf{M}ulti-\textbf{D}omain \textbf{F}usion \textbf{C}hannel \textbf{E}xtrapolator (MDFCE) to extrapolate sub-6 GHz band CSI to mmWave band CSI, so as to reduce the pilot overhead for mmWave CSI acquisition in dual band massive MIMO systems. Unlike traditional channel extrapolation methods based on mathematical modeling, the proposed MDFCE combines the mixture-of-experts framework and the multi-head self-attention mechanism to fuse multi-domain features of sub-6 GHz CSI, aiming to characterize the mapping from sub-6 GHz CSI to mmWave CSI effectively and efficiently. The simulation results demonstrate that MDFCE can achieve superior performance with less training pilots compared with existing methods across various antenna array scales and signal-to-noise ratio levels while showing a much higher computational efficiency.

==> Zhou_WCL2026-1045_table1.tex <==
\begin{table}[b]
    \centering
    \caption{System and hyper-parameter settings.}
    \setlength{\tabcolsep}{3.5pt}
    \begin{tabular}{c|c|c|c}
    \hline
    \multicolumn{4}{c}{\textbf{System settings}} \\
    \hline
    \multicolumn{2}{c|}{ITEM} & \multicolumn{2}{c}{SETTINGS} \\
    \hline
    \multicolumn{2}{c|}{Freq. bands (UL/DL)} & \multicolumn{2}{c}{3.5 GHz / 28 GHz} \\
    \hline
    \multicolumn{2}{c|}{UE antennas (UL/DL)} & \multicolumn{2}{c}{2 / 2} \\
    \hline
    \multicolumn{2}{c|}{BS antennas (UL/DL)} & \multicolumn{2}{c}{4,16 / 8,32} \\
    \hline
    \multicolumn{2}{c|}{Spacing (UL/DL)} & \multicolumn{2}{c}{0.5$\lambda$ / 0.5$\lambda$} \\
    \hline
    \multicolumn{2}{c|}{Bandwidth (UL/DL)} & \multicolumn{2}{c}{40 MHz / 123 MHz} \\
    \hline
    \multicolumn{2}{c|}{Subcarriers (UL/DL)} & \multicolumn{2}{c}{128 / 256} \\
    \hline
    \multicolumn{2}{c|}{Paths (UL/DL)} & \multicolumn{2}{c}{15 / 5} \\
    \hline
    \multicolumn{4}{c}{\textbf{Hyper-parameter settings}} \\
    \hline
    ITEM & SETTINGS & ITEM & SETTINGS \\
    \hline
    Learning rate & $1e-4$ & Epochs & $1000$ \\
    \hline
    Batch size & 128 & Optimizer & AdamW \\
    \hline
    DFIM blocks $N_{s}$ & 7 & Heads $N_{h}$ & 4 \\
    \hline
    Rep. dim. $d_{re}$ & 128 & Hidden dim. $d_{hid}$ & 256 \\
    \hline
    Experts $N_e$ & 8 & Expert dim. $d_{e}$ & $d_{hid}/N_e=32$ \\
    \hline
    Top-K experts $K$ & 2 & Balance factor $\kappa$ & 0.99 \\
    \hline 
    \end{tabular}
    \label{tab:exp-settings}
    \vspace*{-1pt}
\end{table}
